A 3 TOPS/W RISC-V Parallel Cluster for Inference of Fine-Grain Mixed-Precision Quantized Neural Networks

The emerging trend of deploying complex algorithms, such as Deep Neural Networks (DNNs), increasingly poses strict memory and energy efficiency requirements on Internet-of-Things (IoT) end-nodes. Mixed-precision quantization has been proposed as a technique to minimize a DNN's memory footprint and maximize its execution efficiency, with negligible end-to-end precision degradation. In this work, we present a novel hardware and software stack for energy-efficient inference of mixed-precision Quantized Neural Networks (QNNs). We introduce Flex-V, a processor based on the RISC-V Instruction Set Architecture (ISA) that features fused Mac&Load mixed-precision dot product instructions; to avoid the exponential growth of the encoding space due to mixed-precision variants, we encode formats into the Control-Status Registers (CSRs). Flex-V core is integrated into a tightly-coupled cluster of eight processors; in addition, we provide a full framework for the end-to-end deployment of DNNs including a compiler, optimized libraries, and a memory-aware deployment flow. Our results show up to 91.5 MAC/cycle and 3.26 TOPS/W on the cluster, implemented in a commercial 22nm FDX technology, with up to 8.5x speed-up, and an area overhead of only 5.6% with respect to the baseline. To demonstrate the capabilities of the architecture, we benchmark it with end-to-end real-life QNNs, improving performance by 2x - 2.5x with respect to existing solutions using fully flexible programmable processors.

==> text/Introduction.tex <==
\section{Introduction and Related Work} 
\label{intro}
Modern IoT applications require the end-nodes to acquire raw data from sensors, extract ``distilled´´ high-level features by applying near-sensors analytics including state-of-the-art ML and DL algorithms, and transmit this semantically dense information to higher-level nodes through wireless channels. \textcolor{red}{ADD CITATIONS}. The deployment of DL at the extreme-edge of the IoT reduces privacy and security concerns as most of the processing is done in-situ and cuts the off-node transmission power. However, running these models on embedded microcontroller systems pose sever challenges due to limited on-chip memory, power budget and compute capabilities, requiring optimizations on both hardware and software.

A well-established solution to shrink the full-precision DL models to fit the limited storage available on microcontrollers is the adoption of low-bitwidth (8-bits or less) integer arithmetic to represent their parameters, after post-training quantization~\cite{qnn-mixed} or quantization-aware training~\cite{hubara}. These techniques have been proficiently demonstrated on state-of-the-art DNN topologies, adopting symmetric or mixed-precision quantization schemes, reducing the model footprint by \textcolor{red}{XX} with a Top-1 accuracy drop in the range of \textcolor{red}{XX}, not significantly impacting the \textcolor{red}{reliability} of many IoT applications. Banner et al.~\cite{banner} propose a post-training 4-bit quantization method with an accuracy drop of a few percent, while authors of~\cite{qnn-mixed} presented further improvements reducing the memory footprint of DNNs up to 7$\times$ at the cost of an accuracy drop of only 4\%.

Moreover, if well supported by the hardware processing systems, reduced precision integer arithmetic offers more efficient computation compared to the costly floating-points. Low-bitwidth integer formats are widely adopted in custom digital and analog accelerators.
%The execution of complex applications on embedded systems based on microcontrollers (MCUs), which feature stringent constraints on memory size, power consumption, and computing power, imposes aggressive optimizations on both software and hardware. Considering the Internet-of-Things (IoT) scenario, a large share of the energy budget is often consumed for wireless communication to higher-level nodes. Reducing the amount of transmitted raw data is pivotal \textcolor{red}{\ref{}}; one way to achieve this is to communicate processed information instead of raw sensor data. A possible solution can be found in algorithms like Deep Neural Networks (DNNs), which can extract classes or high-level features from data collected by sensors. However, state-of-the-art DNNs rely on a huge number of Multiply-Accumulate (MAC) operations (often in the order of \textcolor{red}{$10^10$}), and their weights have typically a memory footprint in the order of 10-100 MB \textcolor{red}{\ref{}}, impacting power and cost of the overall IoT node.
%
%An effective technique to reduce the memory footprint of DNNs is \textit{quantization}, which reduces activations and weights to low-precision formats employing 8 or less bits \cite{qnn-mixed} - \cite{hubara}, potentially improving their energy efficiency. Banner et al. \cite{banner} propose a post-training 4-bit quantization method with an accuracy drop of a few percent. Rusci et al. \cite{qnn-mixed} presented further improvements reducing the memory footprint of DNNs up to 7$\times$ at the cost of an accuracy drop of only 4\%. However, to efficiently take advantage of quantization during the inference process, proper hardware support is needed. 
%
% HW accelerators
%\subsection{Dedicated hardware accelerators}
% Dedicated hardware accelerators are the best solution in terms of performance and energy efficiency on the QNN workloads. Their highly specialized datapath makes them able to achieve performance in the order of 200 GOPS with energy efficiency in the order of 100 TOPS/W. UNPU \cite{unpu} is an accelerator that supports fully-variable weight bit-precision with a peak efficiency of 50.6 TOPS/W at a throughput of 184 GOPS. DIANA \cite{diana} is a relevant example of a hybrid digital and analog in-memory compute (AiMC) accelerator, the SoC reaches an energy efficiency up to 4.1 TOPS/W when only using the digital core, and 410 TOPS/W when only using the AiMC core. \newline
%A possible solution is to exploit specialized hardware accelerators, which provide the best performance and energy efficiency in exchange for a steep cost in area and flexibility. 
Dedicated digital designs are capable of achieving efficiency in the order of 1-50 TOPS/W depending on the target precision, which might be increased to $>$100 TOPS/W exploiting Analog in-Memory Computing (AiMC). Noticeable examples in this field are: UNPU \cite{unpu}, an accelerator that supports fully-variable weight bit precision from 1 to 16 bit with a peak efficiency of 50.6 TOPS/W at a throughput of 184 GOPS, and DIANA \cite{diana}, a hybrid digital and analog in-memory compute (AiMC) accelerator that reaches an energy efficiency up to 4.1 TOPS/W when only using the digital core, and 410 TOPS/W when only using the AiMC core.
% Despite their energy efficiency, dedicated hardware accelerators lack flexibility while on IoT nodes there's the need to execute several kinds of workloads different from DNNs.
\textcolor{red}{TO BE CONTINUED.....}
Despite their energy efficiency, dedicated hardware accelerators often require a huge area to get efficient for a single specific application, but the constant and ongoing evolution of workloads on IoT nodes requires flexibility.

% FPGAs
%\subsection{FPGAs}
%\noindent
% Heterogeneous FPGAs introduce a higher level of flexibility to build CNN acceleration systems. General purpose processors embedded on FPGA boards can be used as a controller, enabling easier programmability and interaction between different devices and sensors, while the actual CNN acceleration is performed by the DSP-capable hardware.
An intermediate step between dedicated accelerators and fully programmable devices is that of FPGAs, where embedded general-purpose processors can be used as a controller while the actual CNN acceleration is performed by the DSP-capable hardware. In recent literature, several works explore reduced-precision arithmetic, such as those by Qiu \cite{qiu}, Prost \cite{prost} and  Umuroglu \cite{finn}, which however have a power consumption orders-of-magnitude larger than the needs of IoT nodes. %Despite most of the FPGA-based solutions having a power envelope that doesn't meet the constraints of an embedded system,
Lattice proposed the sensAI stack \cite{sensai}, which offers machine learning ultra-low-power capabilities on FPGAs devices with a power envelope between 1 mW and 1 W. However, these have a limited number of LUTs and a non-negligible cost, not compatible with many IoT applications.
%The reconfigurability of these platforms increases the flexibility of the hardware with respect to ASIC solutions, but it is still far from the demand of the average IoT programmer. Additionally, their efficiency is much lower than that offered by ASICs.

% MCUs
%\subsection{Software Programmable solutions}
%\noindent
The highest flexibility for the inference of QNNs is offered by commercial general-purpose processors. The most common kind of programmable embedded systems for ML inference employs high-performance multi-core hardware, such as Raspberry Pi 3+ \cite{raspberry}, or a CPU coupled with an accelerator like Intel Neural Compute Stick 2 \cite{ncs}. Despite their flexibility and relatively low cost, these solutions feature a high power consumption in the order of Watts, not compatible with IoT end-nodes. A recent approach to the enhancement of low-power MCU systems performance consists in the extension of their Instruction Set Architecture (ISA) with dedicated instructions for specific applications.  Many solutions in the RISC-V world leverage this approach, starting from XpulpV2 ISA extensions \cite{ri5cy} for DSP applications, going through MPIC \cite{mpic}, and XpulpNN \cite{xpulpnn}. While MPIC takes advantage of hardware support for mixed-precision operations from 16 to 2 bits, XpulpNN offers fused \textit{Mac\&Load} SIMD instructions for data with symmetric precisions from 16 bits down to 2 bits.

% Contribution
%\subsection{Contribution of this work}
%\noindent
In this work, we present a new hardware and software stack targeting energy-efficient inference of mixed-precision QNNs on a parallel cluster of RISC-V processors. The main contributions of this paper are the following:
\begin{itemize}
    \item We extend the RISC-V ISA with fused mixed-precision \textit{Mac\&Load} instructions. The proposed instruction set extension allows to achieve an ASIC-like utilization of MAC units larger than 80\%, being able to operate on all the mixed-precision variants.
    \item We integrate the extended processor in an eight cores parallel ultra-low-power (PULP) cluster in a commercial 22nm FDX technology to evaluate accurately the impact of such extensions on the operating frequency, area and power of the cluster.
    \item We integrate the proposed hardware extensions in a software framework for end-to-end deployment of DNNs including a compiler, optimized libraries, and a memory-aware deployment flow.
    %\item We compare the extended processor with state-of-the-art architectures by running both single convolutional layers and full end-to-end QNNs.
    \item We compare the extended processor with state-of-the-art architectures by running both single convolutional layers and full end-to-end QNNs. Our results show a performance improvement, with respect to the execution with the extensions disabled, up to 6.8$\times$ on a single layer and up to \textcolor{red}{4}$\times$ on the end-to-end network with negligible degradation of accuracy and a maximum energy efficiency of 4.6 TOPS/W.
\end{itemize}
